Efficient Ensemble Model Generation for Uncertainty Estimation with Bayesian Approximation in Segmentation

Recent studies have shown that ensemble approaches could not only improve accuracy and but also estimate model uncertainty in deep learning. However, it requires a large number of parameters according to the increase of ensemble models for better prediction and uncertainty estimation. To address this issue, a generic and efficient segmentation framework to construct ensemble segmentation models is devised in this paper. In the proposed method, ensemble models can be efficiently generated by using the stochastic layer selection method. The ensemble models are trained to estimate uncertainty through Bayesian approximation. Moreover, to overcome its limitation from uncertain instances, we devise a new pixel-wise uncertainty loss, which improves the predictive performance. To evaluate our method, comprehensive and comparative experiments have been conducted on two datasets. Experimental results show that the proposed method could provide useful uncertainty information by Bayesian approximation with the efficient ensemble model generation and improve the predictive performance.

==> Figure/Figure_4.tex <==
\begin{figure*}[t]
	\centering
	\includegraphics[width=0.95\textwidth]{./Figure/Figure4}
	%\vspace{-0.5cm}
	\caption{Qualitative results of segmentation and uncertainty estimation in our method on TVUS dataset. (a) Original images, (b) is ground truth segmentation images, (c) is segmentation results by the proposed method, (d) is uncertainty map by the proposed method, (e) is difference between ground truth and segmentation results.}
	%\vspace{-0.5cm}
	\label{fig4121}
\end{figure*} 

==> Figure/alg1.tex <==
% \begin{figure}[t]
% 	\centering
% 	\includegraphics[width=0.45\textwidth]{./figure/alg1}
% 	%\vspace{-0.3cm}
% 	%\vspace{-0.5cm}
% 	\label{fig1}
% \end{figure} 

\begin{algorithm}[!t]
	\caption{Pseudocode of the training and the test procedure for our method}

	\label{Alg:1}
	\algsetup{linenosize=\small}
	\small
	\textbf{Training:} For a given training data $X$, training label $Y$, number of sample $N$, and total training iteration $T$ \\
	 ${1}^{st}$ \textbf{step}  \\
	\For{$i=1,2,\cdots ,t$} {
	Select mini-batch set $({{x}_{i}},{{y}_{i}})\sim (X,Y)$ in training dataset \\
    Generate sampled model with ${{P}_{l}}$, \\
    where {P}_{l}\sim categorical({{x}_{1}},{{x}_{2}},...,{{x}_{M}};{{\mu }_{1}},{{\mu }_{2}},...,{{\mu }_{M}}) \\
    Minimize  ${\mathcal{L}_{var}}(x_i,y_i,{{w}_{i}}^{Sample})$, where ${{w}_{i}}^{Sample}$ is the weight of sampled model \\
	}
     ${2}^{nd}$ \textbf{step} \\
	\For{$j=t+1,\cdots ,T$} {Select mini-batch set (${{x}_{i}},{{y}_{i}}$) in training dataset \\
	\For{$n=1, \cdots , N$}{
    Randomly sample prediction $S_n$ with ${{w}_{n}}^{Sample}$}\\
    Estimate uncertainty with sample prediction\\
    $\mathbf{\mathit{S}}=\{{{\hat{S}}_{1}},{{\hat{S}}_{2}},...,{{\hat{S}}_{N}}\}$\\   $\mathbf{\mathit{U}}=var\{{{\hat{S}}_{1}},{{\hat{S}}_{2}},...,{{\hat{S}}_{N}}\}$ \\
    Normalize the $U\sim (0,1)$ \\
    Minimize %Eq. \ref{eq8} 
    ${\mathcal{L}_{total}(x_j,y_j,{{w}_{j}}^{Sample},U)}$ \\
    }
    \\ \hrulefill \\
    \textbf{Test:} For a given test image \textbf{x}\\
    \For{$n=1,\cdots, N$}{
    Randomly sample prediction $S_n$ with ${{w}_{n}}^{Sample}$
    }\\
    Final prediction  $\mathbf{{y}}$=$mean({{\hat{S}}_{1}},{{\hat{S}}_{2}},...,{{\hat{S}}_{N}})$\\
    Estimated uncertainty $\mathbf{{u}}$=$var\{{{\hat{S}}_{1}},{{\hat{S}}_{2}},...,{{\hat{S}}_{N}}\}$
\end{algorithm}

